Learning Causal Orderings for In-Context Tabular Prediction

In-context learning for tabular data sets strong predictive standards in observational settings; it however primarily relies on correlational structure, which becomes unreliable under distribution shift or intervention. While established methods to discover causal structure exist, they are often focused on structure identifiability and decoupled from the predictive architectures that could benefit from them. To bridge these perspectives, we study how to simultaneously infer and enforce causal structure in the form of topological variable orderings into tabular prediction. Unlike standard architectures, our model TabOrder uses causal order-constrained attention, basing predictions only on features that precede a target under a learned causal order. Similar to causal discovery methods, TabOrder learns the optimal variable ordering in an unsupervised manner through a likelihood-based objective. We justify this choice under standard functional model classes and also study how sample missingness, a common challenge in tabular data, interacts with causal direction identification. Empirically, we confirm that TabOrder recovers accurate variable orderings while addressing prediction and imputation tasks, as well as gives insight into real-world biological data under intervention.

==> figs/figs/order-box-synthetic.tex <==
\begin{figure} 

\begin{axis}[ pretty boxplot ]
	\foreach \col in {additive_regularized_gp_small,non_additive_regularized_gp_small,additive_regularized_poly_small,non_additive_unregularized_gp_small,additive_unregularized_poly_small,additive_unregularized_gp_small,rtwosort}{
		\addplot table[y=\col] {texdata/order_box_additive_gp_topological_divergence.tsv};
	}
\end{axis}

\end{figure}

==> figs/full-imputation-table-CC18.tex <==
% Auto-generated from src/results/CC18 (MCAR only)
\begin{longtable}{llrrrrr}
\toprule
Method & Dataset & RMSE 0.1 & RMSE 0.2 & RMSE 0.3 & RMSE 0.4 & RMSE 0.5 \\ 
\midrule
\endfirsthead
\toprule
Method & Dataset & RMSE 0.1 & RMSE 0.2 & RMSE 0.3 & RMSE 0.4 & RMSE 0.5 \\ 
\midrule
\endhead
finetuned-foundation & balance-scale & 0.97 & 0.99 & 0.99 & 1.00 & 1.00 \
finetuned-foundation & breast-w & 0.68 & 0.67 & 0.67 & 0.67 & 0.67 \
finetuned-foundation & mfeat-morphological & 0.26 & 0.34 & 0.44 & 0.53 & 0.63 \
finetuned-foundation & diabetes & 0.77 & 0.83 & 0.85 & 0.87 & 0.89 \
finetuned-foundation & spambase & 0.98 & 0.97 & 0.96 & 0.98 & 0.98 \
finetuned-foundation & vehicle & 0.44 & 0.45 & 0.46 & 0.48 & 0.51 \
finetuned-foundation & electricity & 0.66 & 0.76 & 0.80 & 0.88 & 0.89 \
finetuned-foundation & satimage & 0.34 & 0.33 & 0.33 & 0.34 & 0.35 \
finetuned-foundation & vowel & 0.82 & 0.87 & 0.90 & 0.93 & 0.96 \
finetuned-foundation & analcatdata\_authorship & 0.84 & 0.85 & 0.85 & 0.85 & 0.86 \
finetuned-foundation & pc4 & 0.44 & 0.45 & 0.45 & 0.46 & 0.48 \
finetuned-foundation & pc3 & 0.42 & 0.42 & 0.45 & 0.46 & 0.47 \
finetuned-foundation & jm1 & 0.62 & 0.66 & 0.71 & 0.72 & 0.72 \
finetuned-foundation & kc2 & 0.29 & 0.34 & 0.35 & 0.38 & 0.39 \
finetuned-foundation & kc1 & 0.27 & 0.31 & 0.32 & 0.34 & 0.35 \
finetuned-foundation & pc1 & 0.22 & 0.26 & 0.28 & 0.30 & 0.30 \
finetuned-foundation & wdbc & 0.49 & 0.56 & 0.58 & 0.60 & 0.61 \
finetuned-foundation & phoneme & 0.72 & 0.75 & 0.78 & 0.81 & 0.85 \
finetuned-foundation & qsar-biodeg & 0.63 & 0.67 & 0.67 & 0.69 & 0.73 \
finetuned-foundation & wall-robot-navigation & 0.70 & 0.72 & 0.75 & 0.77 & 0.80 \
finetuned-foundation & ilpd & 0.78 & 0.71 & 0.73 & 0.75 & 0.79 \
finetuned-foundation & ozone-level-8hr & 0.54 & 0.54 & 0.55 & 0.55 & 0.56 \
finetuned-foundation & first-order-theorem-proving & 0.48 & 0.52 & 0.59 & 0.60 & 0.62 \
finetuned-foundation & banknote-authentication & 0.55 & 0.63 & 0.70 & 0.76 & 0.81 \
finetuned-foundation & blood-transfusion-service-center & 0.90 & 0.88 & 0.88 & 0.89 & 0.89 \
finetuned-foundation & GesturePhaseSegmentationProcessed & 0.85 & 0.84 & 0.85 & 0.87 & 0.88 \
finetuned-foundation & MiceProtein & 0.44 & 0.47 & 0.49 & 0.52 & 0.58 \
finetuned-foundation & steel-plates-fault & 0.68 & 0.66 & 0.67 & 0.66 & 0.69 \
finetuned-foundation & climate-model-simulation-crashes & 0.99 & 1.00 & 0.99 & 0.99 & 1.00 \
finetuned-foundation & wilt & 0.85 & 0.81 & 0.79 & 0.79 & 0.79 \
finetuned-foundation & segment & 0.82 & 0.74 & 0.71 & 0.75 & 0.78 \
finetuned-foundation & jungle\_chess\_2pcs\_raw\_endgame\_complete & 0.99 & 0.99 & 0.99 & 1.00 & 1.00 \
finetuned-foundation & churn & 0.89 & 0.88 & 0.89 & 0.91 & 0.93 \
gain & balance-scale & 1.12 & 1.11 & 1.11 & 1.11 & 1.11 \
gain & breast-w & 0.77 & 0.75 & 0.75 & 0.74 & 0.77 \
gain & mfeat-morphological & 0.63 & 0.68 & 0.72 & 0.76 & 0.81 \
gain & diabetes & 0.89 & 0.90 & 0.93 & 0.98 & 1.04 \
gain & spambase & 1.03 & 1.02 & 1.01 & 1.04 & 1.06 \
gain & vehicle & 0.55 & 0.58 & 0.61 & 0.75 & 0.86 \
gain & electricity & 1.29 & 1.45 & 1.58 & 1.61 & 1.62 \
gain & satimage & 0.34 & 0.35 & 0.37 & 0.40 & 0.47 \
gain & vowel & 0.86 & 0.89 & 0.94 & 1.06 & 1.17 \
gain & analcatdata\_authorship & 0.86 & 0.89 & 0.93 & 1.09 & 1.36 \
gain & pc4 & 0.55 & 0.57 & 0.59 & 0.64 & 0.73 \
gain & pc3 & 0.55 & 0.53 & 0.57 & 0.64 & 0.75 \
gain & jm1 & 1.06 & 1.18 & 1.26 & 1.30 & 1.39 \
gain & kc2 & 0.42 & 0.48 & 0.51 & 0.55 & 0.62 \
gain & kc1 & 0.40 & 0.45 & 0.46 & 0.49 & 0.52 \
gain & pc1 & 0.36 & 0.39 & 0.42 & 0.46 & 0.51 \
gain & wdbc & 0.51 & 0.56 & 0.60 & 0.68 & 0.83 \
gain & phoneme & 1.03 & 1.06 & 1.08 & 1.11 & 1.12 \
gain & qsar-biodeg & 0.77 & 0.79 & 0.81 & 1.18 & 1.70 \
gain & wall-robot-navigation & 0.85 & 0.87 & 0.89 & 0.93 & 1.00 \
gain & ilpd & 0.93 & 0.91 & 0.97 & 0.99 & 1.07 \
gain & ozone-level-8hr & 0.51 & 0.52 & 0.53 & 0.81 & 1.18 \
gain & first-order-theorem-proving & 0.68 & 0.70 & 0.77 & 0.85 & 1.22 \
gain & banknote-authentication & 0.95 & 0.92 & 0.98 & 1.03 & 1.05 \
gain & blood-transfusion-service-center & 1.27 & 1.26 & 1.19 & 1.26 & 1.18 \
gain & GesturePhaseSegmentationProcessed & 1.01 & 1.01 & 1.15 & 3.16 & 6.28 \
gain & MiceProtein & 0.43 & 0.48 & 0.52 & 0.69 & 1.09 \
gain & steel-plates-fault & 0.67 & 0.72 & 0.75 & 0.82 & 1.03 \
gain & climate-model-simulation-crashes & 1.19 & 1.15 & 1.15 & 1.17 & 1.23 \
gain & wilt & 1.16 & 1.46 & 1.24 & 1.18 & 1.23 \
gain & segment & 0.90 & 0.87 & 0.90 & 0.98 & 1.15 \
gain & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.14 & 1.13 & 1.13 & 1.14 & 1.16 \
gain & churn & 0.99 & 0.95 & 0.98 & 1.13 & 1.24 \
hyperimpute & balance-scale & 1.03 & 1.04 & 1.08 & 1.12 & 1.13 \
hyperimpute & breast-w & 0.70 & 0.68 & 0.71 & 0.70 & 0.74 \
hyperimpute & mfeat-morphological & 0.41 & 0.48 & 0.55 & 0.63 & 0.72 \
hyperimpute & diabetes & 0.79 & 0.83 & 0.87 & 0.90 & 0.94 \
hyperimpute & spambase & 0.91 & 0.95 & 0.98 & 1.02 &  \
hyperimpute & vehicle & 0.41 & 0.43 & 0.47 & 0.48 & 0.55 \
hyperimpute & electricity & 0.68 & 0.77 & 0.86 & 0.98 & 1.07 \
hyperimpute & satimage & 0.18 & 0.20 & 0.22 & 0.23 & 0.25 \
hyperimpute & vowel & 0.56 & 0.65 & 0.75 & 0.84 & 0.90 \
hyperimpute & analcatdata\_authorship & 0.83 & 0.87 & 0.88 & 0.84 & 0.84 \
hyperimpute & pc4 & 0.32 & 0.33 & 0.39 & 0.41 & 0.51 \
hyperimpute & pc3 & 0.33 & 0.35 & 0.37 & 0.41 & 0.45 \
hyperimpute & jm1 & 0.61 & 0.66 & 0.70 & 0.76 & 0.74 \
hyperimpute & kc2 & 0.30 & 0.41 & 0.43 & 0.46 & 0.52 \
hyperimpute & kc1 & 0.25 & 0.31 & 0.35 & 0.40 & 0.42 \
hyperimpute & pc1 & 0.23 & 0.30 & 0.32 & 0.35 & 0.38 \
hyperimpute & wdbc & 0.30 & 0.39 & 0.43 & 0.49 & 0.54 \
hyperimpute & phoneme & 0.64 & 0.73 & 0.80 & 0.88 & 0.94 \
hyperimpute & wall-robot-navigation & 0.55 & 0.59 & 0.63 & 0.69 & 0.75 \
hyperimpute & ilpd & 0.77 & 0.72 & 0.73 & 0.75 & 0.76 \
hyperimpute & ozone-level-8hr & 0.34 & 0.38 & 0.40 & 0.43 & 0.46 \
hyperimpute & first-order-theorem-proving & 0.33 & 0.38 & 0.45 & 0.49 & 0.53 \
hyperimpute & banknote-authentication & 0.59 & 0.70 & 0.82 & 0.88 & 0.98 \
hyperimpute & blood-transfusion-service-center & 0.95 & 0.93 & 0.93 & 0.94 & 0.96 \
hyperimpute & GesturePhaseSegmentationProcessed & 0.55 & 0.66 & 0.72 & 0.76 & 0.82 \
hyperimpute & MiceProtein & 0.33 & 0.41 & 0.46 & 0.49 & 0.52 \
hyperimpute & climate-model-simulation-crashes & 0.99 & 0.99 & 1.01 & 1.02 & 1.05 \
hyperimpute & wilt & 0.87 & 0.82 & 0.81 & 0.82 & 0.84 \
hyperimpute & segment & 0.74 & 0.71 & 0.72 & 0.74 & 0.81 \
hyperimpute & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.00 & 1.03 & 1.09 & 1.14 & 1.19 \
hyperimpute & churn & 0.87 & 0.87 & 0.88 & 0.88 & 0.95 \
ice & balance-scale & 1.02 & 1.02 & 1.02 & 1.04 & 1.07 \
ice & breast-w & 0.74 & 0.71 & 0.73 & 0.77 & 0.78 \
ice & mfeat-morphological & 0.45 & 0.52 & 0.60 & 0.66 & 0.74 \
ice & diabetes & 0.81 & 0.85 & 0.90 & 0.98 & 1.01 \
ice & spambase & 0.95 & 0.96 & 1.11 & 1.17 & 1.17 \
ice & vehicle & 0.42 & 0.44 & 0.47 & 0.51 & 0.55 \
ice & electricity & 0.91 & 0.93 & 0.99 & 1.01 & 1.03 \
ice & satimage & 0.18 & 0.20 & 0.23 & 0.25 & 0.28 \
ice & vowel & 0.70 & 0.77 & 0.82 & 0.87 & 0.91 \
ice & analcatdata\_authorship & 0.82 & 1.02 & 1.04 & 1.01 & 1.00 \
ice & pc4 & 0.41 & 0.49 & 0.54 & 0.54 & 0.59 \
ice & pc3 & 0.34 & 0.37 & 0.42 & 0.46 & 0.50 \
ice & jm1 & 0.61 & 0.65 & 0.73 & 0.79 & 0.77 \
ice & kc2 & 0.32 & 0.41 & 0.43 & 0.47 & 0.52 \
ice & kc1 & 0.26 & 0.35 & 0.40 & 0.44 & 0.45 \
ice & pc1 & 0.24 & 0.46 & 0.34 & 0.42 & 0.43 \
ice & wdbc & 0.30 & 0.39 & 0.45 & 0.51 & 0.55 \
ice & phoneme & 0.92 & 0.94 & 0.96 & 1.00 & 1.01 \
ice & qsar-biodeg & 0.49 & 0.60 & 0.70 & 0.76 & 0.85 \
ice & wall-robot-navigation & 0.77 & 0.79 & 0.89 & 0.93 & 0.92 \
ice & ilpd & 0.75 & 0.77 & 0.76 & 0.78 & 0.79 \
ice & ozone-level-8hr & 0.34 & 0.40 & 0.46 & 0.48 & 0.51 \
ice & first-order-theorem-proving & 0.43 & 0.53 & 0.57 & 0.58 & 0.64 \
ice & banknote-authentication & 0.79 & 0.81 & 0.84 & 0.88 & 0.92 \
ice & blood-transfusion-service-center & 0.97 & 0.95 & 1.01 & 0.92 & 1.06 \
ice & GesturePhaseSegmentationProcessed & 0.59 & 0.69 & 0.73 & 0.78 & 0.83 \
ice & MiceProtein & 0.33 & 0.43 & 0.50 & 0.53 & 0.54 \
ice & steel-plates-fault & 0.45 & 0.52 & 0.56 & 0.62 & 0.69 \
ice & climate-model-simulation-crashes & 1.01 & 1.02 & 1.21 & 1.27 & 1.25 \
ice & wilt & 0.87 & 0.83 & 0.86 & 1.07 & 0.85 \
ice & segment & 0.95 & 0.97 & 0.99 & 1.13 & 1.15 \
ice & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.00 & 1.00 & 1.00 & 1.00 & 1.09 \
ice & churn & 0.84 & 0.83 & 0.83 & 0.87 & 1.00 \
knn & balance-scale & 1.14 & 1.13 & 1.11 & 1.10 & 1.08 \
knn & breast-w & 0.76 & 0.77 & 0.79 & 0.79 & 0.79 \
knn & mfeat-morphological & 0.46 & 0.67 & 0.78 & 0.83 & 0.84 \
knn & diabetes & 0.86 & 0.93 & 0.97 & 0.97 & 0.98 \
knn & spambase & 0.94 & 0.98 & 1.03 & 1.07 & 1.15 \
knn & vehicle & 0.44 & 0.46 & 0.50 & 0.55 & 0.66 \
knn & electricity & 0.79 & 0.92 & 1.03 & 1.04 & 1.03 \
knn & satimage & 0.22 & 0.24 & 0.25 & 0.29 & 0.36 \
knn & vowel & 0.50 & 0.63 & 0.79 & 0.92 & 0.99 \
knn & analcatdata\_authorship & 0.84 & 0.86 & 0.87 & 0.89 & 0.91 \
knn & pc4 & 0.43 & 0.46 & 0.49 & 0.51 & 0.57 \
knn & pc3 & 0.45 & 0.46 & 0.48 & 0.50 & 0.54 \
knn & jm1 & 0.70 & 0.78 & 0.90 & 1.06 & 1.08 \
knn & kc2 & 0.44 & 0.58 & 0.59 & 0.61 & 0.67 \
knn & kc1 & 0.27 & 0.31 & 0.33 & 0.41 & 0.54 \
knn & pc1 & 0.26 & 0.30 & 0.32 & 0.35 & 0.42 \
knn & wdbc & 0.53 & 0.58 & 0.64 & 0.68 & 0.74 \
knn & phoneme & 0.70 & 0.83 & 0.87 & 0.90 & 0.91 \
knn & qsar-biodeg & 0.57 & 0.63 & 0.69 & 0.74 & 0.87 \
knn & wall-robot-navigation & 0.60 & 0.61 & 0.62 & 0.63 & 0.72 \
knn & ilpd & 0.90 & 0.89 & 0.89 & 0.91 & 0.93 \
knn & ozone-level-8hr & 0.50 & 0.51 & 0.53 & 0.55 & 0.59 \
knn & first-order-theorem-proving & 0.42 & 0.46 & 0.52 & 0.55 & 0.62 \
knn & banknote-authentication & 0.71 & 0.84 & 0.90 & 0.92 & 0.93 \
knn & blood-transfusion-service-center & 1.06 & 1.03 & 0.99 & 1.00 & 1.00 \
knn & GesturePhaseSegmentationProcessed & 0.74 & 0.83 & 0.91 & 0.97 & 1.02 \
knn & MiceProtein & 0.38 & 0.42 & 0.45 & 0.49 & 0.53 \
knn & steel-plates-fault & 0.49 & 0.56 & 0.61 & 0.68 & 0.79 \
knn & climate-model-simulation-crashes & 1.07 & 1.09 & 1.08 & 1.09 & 1.09 \
knn & wilt & 0.96 & 0.93 & 0.91 & 0.90 & 0.89 \
knn & segment & 0.80 & 0.79 & 0.82 & 0.93 & 1.09 \
knn & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.10 & 1.09 & 1.10 & 1.09 & 1.09 \
knn & churn & 0.98 & 1.00 & 1.03 & 1.06 & 1.08 \
mean & balance-scale & 1.01 & 1.01 & 1.01 & 1.01 & 1.01 \
mean & breast-w & 1.01 & 1.00 & 1.01 & 0.99 & 0.99 \
mean & mfeat-morphological & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 \
mean & diabetes & 0.92 & 0.93 & 0.93 & 0.93 & 0.93 \
mean & spambase & 1.05 & 1.05 & 1.07 & 1.07 & 1.08 \
mean & vehicle & 1.02 & 1.01 & 1.00 & 1.00 & 1.00 \
mean & electricity & 1.06 & 1.06 & 1.10 & 1.08 & 1.06 \
mean & satimage & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 \
mean & vowel & 0.99 & 0.99 & 0.99 & 1.00 & 1.00 \
mean & analcatdata\_authorship & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \
mean & pc4 & 0.76 & 0.76 & 0.77 & 0.76 & 0.77 \
mean & pc3 & 0.79 & 0.77 & 0.76 & 0.75 & 0.75 \
mean & jm1 & 1.19 & 1.16 & 1.18 & 1.22 & 1.17 \
mean & kc2 & 0.90 & 1.02 & 1.00 & 0.99 & 0.99 \
mean & kc1 & 0.87 & 0.88 & 0.88 & 0.88 & 0.88 \
mean & pc1 & 0.60 & 0.61 & 0.61 & 0.60 & 0.60 \
mean & wdbc & 1.02 & 1.04 & 1.04 & 1.04 & 1.04 \
mean & phoneme & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \
mean & qsar-biodeg & 1.00 & 1.00 & 0.99 & 0.98 & 1.00 \
mean & wall-robot-navigation & 0.98 & 0.99 & 0.99 & 0.99 & 0.99 \
mean & ilpd & 0.94 & 0.91 & 0.90 & 0.89 & 0.89 \
mean & ozone-level-8hr & 1.00 & 1.01 & 1.01 & 1.01 & 1.01 \
mean & first-order-theorem-proving & 1.00 & 1.00 & 1.01 & 1.00 & 1.00 \
mean & banknote-authentication & 1.01 & 1.01 & 1.02 & 1.03 & 1.04 \
mean & blood-transfusion-service-center & 1.16 & 1.14 & 1.12 & 1.13 & 1.13 \
mean & GesturePhaseSegmentationProcessed & 1.02 & 1.01 & 1.02 & 1.02 & 1.02 \
mean & MiceProtein & 0.99 & 0.99 & 1.00 & 1.00 & 1.00 \
mean & steel-plates-fault & 0.99 & 0.98 & 0.97 & 0.97 & 0.97 \
mean & climate-model-simulation-crashes & 0.98 & 0.98 & 0.99 & 0.99 & 1.00 \
mean & wilt & 0.90 & 0.89 & 0.88 & 0.87 & 0.86 \
mean & segment & 1.09 & 1.11 & 1.14 & 1.14 & 1.16 \
mean & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \
mean & churn & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \
mice & balance-scale & 1.42 & 1.43 & 1.42 & 1.41 & 1.45 \
mice & breast-w & 1.01 & 0.98 & 0.98 & 0.96 & 0.97 \
mice & mfeat-morphological & 0.57 & 0.66 & 0.77 & 0.84 & 0.94 \
mice & diabetes & 1.19 & 1.24 & 1.24 & 1.27 & 1.29 \
mice & spambase & 1.32 & 1.31 & 1.33 & 1.35 & 1.38 \
mice & vehicle & 0.59 & 0.60 & 0.62 & 0.65 & 0.69 \
mice & electricity & 1.25 & 1.27 & 1.32 & 1.34 & 1.34 \
mice & satimage &  & 0.27 &  & 0.30 & 0.33 \
mice & vowel & 0.99 & 1.08 & 1.13 & 1.20 & 1.24 \
mice & analcatdata\_authorship & 1.13 & 1.15 & 1.17 & 1.19 & 1.20 \
mice & pc4 & 0.62 & 0.63 & 0.66 & 0.68 &  \
mice & pc3 & 0.51 & 0.55 & 0.58 & 0.62 & 0.70 \
mice & jm1 & 0.67 & 0.70 & 0.72 & 0.81 & 0.81 \
mice & kc2 & 0.44 & 0.52 & 0.55 & 0.64 & 0.68 \
mice & kc1 & 0.42 & 0.53 & 0.55 & 0.59 & 0.61 \
mice & pc1 &  & 1.01 & 0.59 & 0.60 & 0.57 \
mice & wdbc & 0.40 & 0.48 & 0.52 & 0.58 & 0.64 \
mice & phoneme & 1.33 & 1.33 & 1.35 & 1.37 & 1.38 \
mice & qsar-biodeg & 0.71 & 0.76 & 0.80 & 0.87 & 0.94 \
mice & wall-robot-navigation & 1.12 & 1.14 & 1.16 & 1.18 & 1.20 \
mice & ilpd & 1.15 & 1.06 & 1.06 & 1.06 & 1.10 \
mice & ozone-level-8hr & 0.47 & 0.49 & 0.51 & 0.53 & 0.57 \
mice & first-order-theorem-proving & 0.57 & 0.61 & 0.67 & 0.73 & 0.79 \
mice & banknote-authentication & 1.11 & 1.15 & 1.17 & 1.21 & 1.23 \
mice & blood-transfusion-service-center & 1.31 & 1.26 & 1.21 & 1.23 & 1.24 \
mice & GesturePhaseSegmentationProcessed & 0.82 & 0.90 & 0.97 & 1.04 & 1.10 \
mice & MiceProtein & 0.46 & 0.50 & 0.54 & 0.58 & 0.63 \
mice & steel-plates-fault & 0.61 & 0.67 & 0.74 & 0.78 & 0.85 \
mice & climate-model-simulation-crashes & 1.39 & 1.40 & 1.42 & 1.41 & 1.42 \
mice & wilt & 1.27 & 1.21 & 1.20 & 1.19 & 1.20 \
mice & segment & 1.07 & 0.99 & 0.98 & 1.00 & 1.04 \
mice & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.42 & 1.41 & 1.42 & 1.42 & 1.41 \
mice & churn & 1.18 & 1.15 & 1.14 & 1.17 & 1.20 \
missforest & balance-scale & 1.03 & 1.04 & 1.05 & 1.06 & 1.08 \
missforest & breast-w & 0.70 & 0.68 & 0.68 & 0.67 & 0.69 \
missforest & mfeat-morphological & 0.38 & 0.46 & 0.54 & 0.63 & 0.72 \
missforest & diabetes & 0.79 & 0.83 & 0.86 & 0.89 & 0.92 \
missforest & spambase & 0.93 & 0.93 & 0.96 & 0.98 & 1.00 \
missforest & vehicle & 0.48 & 0.48 & 0.49 & 0.49 & 0.53 \
missforest & electricity & 0.70 & 0.74 & 0.85 & 0.90 & 0.91 \
missforest & satimage & 0.30 & 0.30 & 0.31 & 0.32 & 0.33 \
missforest & vowel & 0.77 & 0.79 & 0.82 & 0.86 & 0.90 \
missforest & analcatdata\_authorship & 0.84 & 0.84 & 0.84 & 0.84 & 0.84 \
missforest & pc4 & 0.40 & 0.44 & 0.46 & 0.48 & 0.51 \
missforest & pc3 & 0.43 & 0.43 & 0.44 & 0.45 & 0.46 \
missforest & jm1 & 0.67 & 0.67 & 0.70 & 0.76 & 0.73 \
missforest & kc2 & 0.31 & 0.42 & 0.44 & 0.46 & 0.48 \
missforest & kc1 & 0.29 & 0.32 & 0.34 & 0.37 & 0.38 \
missforest & pc1 & 0.26 & 0.30 & 0.31 & 0.32 & 0.34 \
missforest & wdbc & 0.51 & 0.55 & 0.58 & 0.59 & 0.62 \
missforest & phoneme & 0.77 & 0.81 & 0.85 & 0.91 & 0.96 \
missforest & qsar-biodeg & 0.60 & 0.65 & 0.66 & 0.68 & 0.74 \
missforest & wall-robot-navigation & 0.70 & 0.73 & 0.75 & 0.77 & 0.80 \
missforest & ilpd & 0.78 & 0.75 & 0.74 & 0.76 & 0.79 \
missforest & ozone-level-8hr & 0.48 & 0.49 & 0.49 & 0.50 & 0.51 \
missforest & first-order-theorem-proving & 0.51 & 0.55 & 0.58 & 0.59 & 0.61 \
missforest & banknote-authentication & 0.76 & 0.77 & 0.82 & 0.86 & 0.91 \
missforest & blood-transfusion-service-center & 0.95 & 0.94 & 0.93 & 0.96 & 0.98 \
missforest & GesturePhaseSegmentationProcessed & 0.83 & 0.84 & 0.85 & 0.86 & 0.88 \
missforest & MiceProtein & 0.51 & 0.54 & 0.57 & 0.58 & 0.60 \
missforest & steel-plates-fault & 0.56 & 0.59 & 0.60 & 0.62 & 0.66 \
missforest & climate-model-simulation-crashes & 0.99 & 0.99 & 1.01 & 1.02 & 1.05 \
missforest & wilt & 0.86 & 0.82 & 0.80 & 0.81 & 0.83 \
missforest & segment & 0.74 & 0.72 & 0.72 & 0.73 & 0.76 \
missforest & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.00 & 1.01 & 1.02 & 1.04 & 1.06 \
missforest & churn & 0.93 & 0.93 & 0.93 & 0.95 & 0.97 \
miwae & balance-scale & 1.09 & 1.13 & 1.10 & 1.12 & 1.12 \
miwae & breast-w & 1.09 & 1.00 & 1.03 & 1.07 & 1.09 \
miwae & mfeat-morphological & 1.01 & 0.95 & 0.96 & 1.02 & 1.03 \
miwae & diabetes & 1.01 & 1.03 & 1.00 & 1.00 & 1.00 \
miwae & spambase & 1.12 & 1.18 & 1.13 & 1.15 & 1.14 \
miwae & vehicle & 0.99 & 1.04 & 0.99 & 1.05 & 1.01 \
miwae & electricity & 1.12 & 1.12 & 1.22 & 1.26 & 1.32 \
miwae & satimage & 1.08 & 1.11 & 1.04 & 1.06 & 1.11 \
miwae & vowel & 1.06 & 1.05 & 1.06 & 1.06 & 1.07 \
miwae & analcatdata\_authorship & 1.12 & 1.12 & 1.11 & 1.11 & 1.10 \
miwae & pc4 & 0.84 & 0.85 & 0.86 & 0.83 & 0.85 \
miwae & pc3 & 0.86 & 0.85 & 0.84 & 0.82 & 0.81 \
miwae & jm1 & 1.24 & 1.20 & 1.34 & 1.28 & 1.32 \
miwae & kc2 & 0.92 & 1.05 & 1.06 & 1.00 & 1.02 \
miwae & kc1 & 0.88 & 0.91 & 0.89 & 0.93 & 0.92 \
miwae & pc1 & 0.60 & 0.62 & 0.62 & 0.62 & 0.60 \
miwae & wdbc & 1.09 & 1.15 & 1.12 & 1.11 & 1.11 \
miwae & phoneme & 1.06 & 1.04 & 1.06 & 1.06 & 1.07 \
miwae & qsar-biodeg & 1.09 & 1.11 & 1.07 & 1.07 & 1.12 \
miwae & wall-robot-navigation & 1.15 & 1.14 & 1.13 & 1.12 & 1.12 \
miwae & ilpd & 1.15 & 1.02 & 1.01 & 1.00 & 0.99 \
miwae & ozone-level-8hr & 1.08 & 1.05 & 1.05 & 1.07 & 1.02 \
miwae & first-order-theorem-proving & 1.13 & 1.13 & 1.14 & 1.13 & 1.12 \
miwae & banknote-authentication & 1.05 & 1.08 & 1.05 & 1.07 & 1.09 \
miwae & blood-transfusion-service-center & 1.25 & 1.22 & 1.20 & 1.19 & 1.19 \
miwae & GesturePhaseSegmentationProcessed & 1.23 & 1.21 & 1.19 & 1.12 & 1.18 \
miwae & MiceProtein & 1.12 & 1.12 & 1.12 & 1.15 & 1.11 \
miwae & steel-plates-fault & 1.10 & 1.12 & 1.09 & 1.06 & 1.08 \
miwae & climate-model-simulation-crashes & 1.11 & 1.10 & 1.10 & 1.10 & 1.11 \
miwae & wilt & 1.03 & 0.97 & 0.96 & 0.94 & 0.93 \
miwae & segment & 1.09 & 1.11 & 1.16 & 1.18 & 1.21 \
miwae & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.06 & 1.07 & 1.06 & 1.06 & 1.06 \
miwae & churn & 1.15 & 1.09 & 1.09 & 1.08 & 1.10 \
pretrained-foundation & balance-scale & 1.19 & 1.23 & 1.21 & 1.22 & 1.24 \
pretrained-foundation & breast-w & 0.81 & 0.84 & 0.86 & 0.89 & 0.93 \
pretrained-foundation & mfeat-morphological & 0.59 & 0.72 & 0.83 & 0.91 & 1.00 \
pretrained-foundation & diabetes & 1.03 & 1.06 & 1.07 & 1.09 & 1.10 \
pretrained-foundation & spambase & 1.58 & 1.26 & 1.18 & 1.18 & 1.18 \
pretrained-foundation & vehicle & 0.60 & 0.64 & 0.72 & 0.80 & 0.89 \
pretrained-foundation & electricity & 0.95 & 1.05 & 1.10 & 1.18 & 1.19 \
pretrained-foundation & satimage & 0.59 & 0.64 & 0.72 & 0.81 & 0.90 \
pretrained-foundation & vowel & 0.96 & 1.00 & 1.05 & 1.10 & 1.13 \
pretrained-foundation & analcatdata\_authorship & 1.02 & 1.03 & 1.03 & 1.04 & 1.06 \
pretrained-foundation & pc4 & 0.80 & 0.87 & 0.93 & 0.95 & 0.95 \
pretrained-foundation & pc3 & 0.83 & 0.87 & 0.88 & 0.88 & 0.89 \
pretrained-foundation & jm1 & 1.06 & 1.11 & 1.27 & 1.31 & 1.36 \
pretrained-foundation & kc2 & 0.77 & 0.82 & 0.90 & 0.96 & 1.04 \
pretrained-foundation & kc1 & 0.60 & 0.70 & 0.85 & 0.92 & 1.00 \
pretrained-foundation & pc1 & 0.57 & 0.61 & 0.78 & 0.88 & 0.97 \
pretrained-foundation & wdbc & 0.72 & 0.86 & 0.93 & 0.99 & 1.03 \
pretrained-foundation & phoneme & 0.97 & 1.02 & 1.05 & 1.09 & 1.12 \
pretrained-foundation & qsar-biodeg & 1.20 & 1.09 & 1.08 & 1.11 & 1.12 \
pretrained-foundation & wall-robot-navigation & 0.99 & 1.02 & 1.04 & 1.12 & 1.14 \
pretrained-foundation & ilpd & 1.09 & 1.02 & 0.99 & 1.00 & 1.03 \
pretrained-foundation & ozone-level-8hr & 0.79 & 0.87 & 0.93 & 0.98 & 1.02 \
pretrained-foundation & first-order-theorem-proving & 1.09 & 1.01 & 1.06 & 1.08 & 1.10 \
pretrained-foundation & banknote-authentication & 0.79 & 0.88 & 0.95 & 1.04 & 1.11 \
pretrained-foundation & blood-transfusion-service-center & 1.18 & 1.17 & 1.20 & 1.24 & 1.29 \
pretrained-foundation & GesturePhaseSegmentationProcessed & 1.21 & 1.20 & 1.16 & 1.16 & 1.16 \
pretrained-foundation & MiceProtein & 0.84 & 0.91 & 1.01 & 1.07 & 1.10 \
pretrained-foundation & steel-plates-fault & 1.01 & 0.97 & 0.97 & 1.01 & 1.05 \
pretrained-foundation & climate-model-simulation-crashes & 1.09 & 1.10 & 1.09 & 1.10 & 1.13 \
pretrained-foundation & wilt & 1.17 & 1.12 & 1.13 & 1.11 & 1.12 \
pretrained-foundation & segment & 1.07 & 1.00 & 1.02 & 1.06 & 1.11 \
pretrained-foundation & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.11 & 1.14 & 1.14 & 1.14 & 1.16 \
pretrained-foundation & churn & 1.12 & 1.11 & 1.13 & 1.15 & 1.16 \
softimpute & balance-scale & 1.01 & 1.01 & 1.01 & 1.01 & 1.01 \
softimpute & breast-w & 0.80 & 0.79 & 0.79 & 0.82 & 0.82 \
softimpute & mfeat-morphological & 0.59 & 0.71 & 0.79 & 0.80 & 0.82 \
softimpute & diabetes & 0.94 & 0.92 & 0.92 & 0.93 & 0.93 \
softimpute & spambase & 0.99 & 1.00 & 1.04 & 1.06 & 1.07 \
softimpute & vehicle & 0.54 & 0.54 & 0.55 & 0.56 & 0.60 \
softimpute & electricity & 1.33 & 1.05 & 1.08 & 1.07 & 1.06 \
softimpute & satimage & 0.42 & 0.42 & 0.42 & 0.42 & 0.42 \
softimpute & vowel & 0.94 & 0.95 & 0.98 & 1.02 & 1.00 \
softimpute & analcatdata\_authorship & 0.89 & 0.89 & 0.88 & 0.89 & 0.89 \
softimpute & pc4 & 0.61 & 0.62 & 0.62 & 0.63 & 0.64 \
softimpute & pc3 & 0.61 & 0.61 & 0.61 & 0.61 & 0.62 \
softimpute & jm1 & 0.70 & 0.78 & 0.79 & 0.85 & 0.84 \
softimpute & kc2 & 0.37 & 0.49 & 0.56 & 0.51 & 1.21 \
softimpute & kc1 & 0.37 & 0.41 & 0.44 & 0.47 & 0.50 \
softimpute & pc1 & 0.34 & 0.38 & 0.59 & 0.41 & 0.42 \
softimpute & wdbc & 0.60 & 0.64 & 0.67 & 0.69 & 0.70 \
softimpute & phoneme & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \
softimpute & qsar-biodeg & 0.85 & 0.87 & 0.86 & 0.87 & 0.93 \
softimpute & wall-robot-navigation & 0.85 & 0.87 & 0.88 & 0.90 & 0.92 \
softimpute & ilpd & 0.81 & 0.79 & 0.89 & 0.88 & 0.88 \
softimpute & ozone-level-8hr & 0.64 & 0.64 & 0.64 & 0.64 & 0.64 \
softimpute & first-order-theorem-proving & 0.81 & 0.82 & 0.83 & 0.84 & 0.85 \
softimpute & banknote-authentication & 0.95 & 0.94 & 0.94 & 0.95 & 0.97 \
softimpute & blood-transfusion-service-center & 1.11 & 1.05 & 0.99 & 1.00 & 1.00 \
softimpute & GesturePhaseSegmentationProcessed & 0.95 & 0.95 & 0.96 & 0.97 & 0.99 \
softimpute & MiceProtein & 0.75 & 0.76 & 0.77 & 0.78 & 0.78 \
softimpute & steel-plates-fault & 0.80 & 0.80 & 0.96 & 0.96 & 0.82 \
softimpute & climate-model-simulation-crashes & 0.98 & 0.98 & 0.99 & 0.99 & 1.00 \
softimpute & wilt & 0.90 & 0.88 & 0.87 & 0.87 & 0.86 \
softimpute & segment & 0.86 & 0.85 & 0.85 & 0.87 & 0.95 \
softimpute & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \
softimpute & churn & 0.98 & 0.99 & 0.99 & 0.99 & 1.00 \
tabimpute & balance-scale & 1.02 & 1.02 & 1.03 & 1.03 & 1.03 \
tabimpute & breast-w & 0.86 & 0.83 & 0.80 & 0.80 & 0.82 \
tabimpute & mfeat-morphological & 0.71 & 0.72 & 0.75 & 0.78 & 0.83 \
tabimpute & diabetes & 0.87 & 0.91 & 0.91 & 0.92 & 0.92 \
tabimpute & electricity & 0.94 & 1.01 & 0.99 & 1.07 & 1.05 \
tabimpute & vowel & 0.89 & 0.92 & 0.94 & 0.97 & 0.99 \
tabimpute & phoneme & 1.01 & 1.01 & 1.01 & 1.00 & 1.01 \
tabimpute & ilpd & 0.97 & 1.01 & 0.99 & 0.95 & 0.96 \
tabimpute & banknote-authentication & 0.90 & 0.92 & 0.94 & 0.95 & 0.96 \
tabimpute & blood-transfusion-service-center & 1.07 & 1.02 & 1.01 & 0.99 & 1.00 \
tabimpute & wilt & 0.93 & 0.91 & 0.89 & 0.88 & 0.87 \
tabimpute & jungle\_chess\_2pcs\_raw\_endgame\_complete & 1.03 & 1.03 & 1.03 & 1.03 & 1.03 \
\bottomrule
\end{longtable}


==> figs/order-heat.tex <==
\pgfplotsset{
	colormap={mycolors}{
		rgb255(0cm)=(255,255,255)
		rgb255(1cm)=(189,215,231)
		rgb255(2cm)=(107,174,214)
	 %	rgb255(2cm)=( 33,113,181)
	%	rgb255(3cm)=(  8, 48,107)
		%rgb255(4cm)=(255,255,255)
		%rgb255(5cm)=(253,187,132)
	%	rgb255(6cm)=(227, 74, 51)
	%	rgb255(7cm)=(179,  0,  0)
	}
}

\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[
	height=4cm, width=5.5cm,
pretty heatmatrix, pretty labelshift,
xtick = {0,1,2,3,4,5},
ytick = {0,1,2},  colormap name=mycolors,
xticklabels = {\textsc{Spline*},\textsc{GP*},\textsc{Mixed*}, \textsc{Spline},\textsc{Mixed},\textsc{GP} },%{spline-lo1,gp-lo1,general-lo1,spline-lo0,general-lo0,gp-lo0},
  xticklabel style={
	rotate=45,        % or 60 / 90
	anchor=east,      % keeps them “hanging” nicely
	align=right
}, 
yticklabels = {\footnotesize \textsc{GP-Additive}, \footnotesize \textsc{GP-NonAdditive}, \footnotesize\textsc{Spline-Additive}},
xlabel = {\ourmethod model},
ylabel = {data generator},
colorbar style = { ylabel = {$\divtop$}, %ymax= 1
},
]
\addplot[pr-matrix, mesh/cols=6] table [meta=z] {figs/texdata/heat_topological_divergence_median.txt};
\end{axis}
\end{tikzpicture}
 \caption{Shown are the effects of (a) training \ourmethod on specific functional forms (spline, Gaussian process, or a mix of functional forms), and of (b) including additional loss supervision given the true causal orders (where * denotes supervised variants). (a) A mix of generating processes (mixed) allows the model to generally fit the data-generating process well compared to specialized (spline, GP) models. (b) While training with explicit supervision (*) further reduces $\divtop$, it may be prone to overfitting the synthetic data generators and, as shown in Figures \ref{fig:full_causal_plot}, is not necessary to achieve competitive performance with the causal discovery baselines, hence we report the main variant (without *) as our main method. 
 }
\label{fig:order_heat}
\end{figure}


==> figs/sachs-flip-graph.tex <==
\begin{figure}[t]
	\centering
	
	% Row 1
%	\begin{subfigure}{0.32\linewidth}
%		\centering
%		\ResetSachsInterventions
%%		\ShowSachsActivatorOne
%		\ShowSachsFlipsCdThreeCdTwentyEight
%		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28}}{0.206}}
%		\caption{\textbf{\texttt{cd3cd28}.}}
%	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsActivatorTwo
		\ShowSachsFlipsICAM
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28\_icam2}}{0.235}}
		\caption{\textbf{\texttt{cd3cd28\_icam2}.} }
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsActivatorThree
		\ShowSachsFlipsPMA
		\scalebox{0.5}{\SachsFlipGraph{\texttt{pma}}{--}}
		\caption{\textbf{\texttt{pma}.} }
	\end{subfigure}
	 \hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSix
		\ShowSachsFlipsUzero
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28\_u0126}}{0.265}}
		\caption{\textbf{\texttt{cd3cd28\_u0126}.} }
	\end{subfigure} 
\vspace{0.7em}
% Row 2
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSix
		\ShowSachsActivatorTwo
		\ShowSachsFlipsICAMUzero
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28icam2\_u0126}}{--}}
		\caption{\textbf{\texttt{cd3cd28icam2\_u0126}.} }
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFive
		\ShowSachsFlipsAktInhib
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28\_aktinhib}}{0.294}}
		\caption{\textbf{\texttt{cd3cd28\_aktinhib}.} }
	\end{subfigure} 
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFive
		\ShowSachsActivatorTwo
		\ShowSachsFlipsICAMAktInhib
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28icam2\_aktinhib}}{0.132}}
		\caption{\textbf{\texttt{cd3cd28icam2\_aktinhib}.} }
	\end{subfigure} 
\vspace{0.7em}  
% Row 3
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFour
		\ShowSachsFlipsGzero
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28\_g0076}}{0.765}}
		\caption{\textbf{\texttt{cd3cd28\_g0076}.} }
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFour
		\ShowSachsActivatorTwo
		\ShowSachsFlipsICAMGzero
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28icam2\_g0076}}{0.544}}
		\caption{\textbf{\texttt{cd3cd28icam2\_g0076}.} }
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSeven
		\ShowSachsFlipsLy
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28\_ly}}{0.191}}
		\caption{\textbf{\texttt{cd3cd28\_ly}.} }
	\end{subfigure} 
	\vspace{0.7em} 
	% Row 4
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSeven
		\ShowSachsActivatorTwo
		\ShowSachsFlipsICAMLy
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28icam2\_ly}}{--}}
		\caption{\textbf{\texttt{cd3cd28icam2\_ly}.} }
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorEight
		\ShowSachsFlipsPsitect
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28\_psitect}}{0.235}}
		\caption{\textbf{\texttt{cd3cd28\_psitect}.} }
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorEight
		\ShowSachsActivatorTwo
		\ShowSachsFlipsICAMPsit
		\scalebox{0.5}{\SachsFlipGraph{\texttt{cd3cd28icam2\_psit}}{--}}
		\caption{\textbf{\texttt{cd3cd28icam2\_psit}.} }
	\end{subfigure}
	
	\caption{\textbf{Differences in causal-order positionings under Sachs experimental conditions.}
		Nodes are colored by pairwise flip fraction relative to \texttt{cd3cd28}; edges show the fixed consensus graph. Activator and inhibitor markers indicate the corresponding experimental perturbations. Panel titles report the global topological divergence $\divtop$ for \ourmethod where available.}
	\label{fig:sachs-all-intervention-graph-flips}
\end{figure}

\begin{figure}[t]
	\centering
	
	\begin{subfigure}{0.48\linewidth}
		\centering
		\scalebox{0.78}{\OrderPanel{\texttt{u0126}}{0.265}{\BaselineOrder}{\OrderUzero}}
		\caption{MEK inhibition}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.48\linewidth}
		\centering
		\scalebox{0.78}{\OrderPanel{\texttt{g0076}}{0.765}{\BaselineOrder}{\OrderGzero}}
		\caption{PKC inhibition}
	\end{subfigure}
	
	\vspace{0.8em}
	
	\begin{subfigure}{0.48\linewidth}
		\centering
		\scalebox{0.78}{\OrderPanel{\texttt{psitect}}{0.235}{\BaselineOrder}{\OrderPsitect}}
		\caption{Phosphoinositide perturbation}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.48\linewidth}
		\centering
		\scalebox{0.78}{\OrderPanel{\texttt{ly}}{0.191}{\BaselineOrder}{\OrderLy}}
		\caption{PI3K inhibition}
	\end{subfigure}
	
	\caption{\textbf{Order changes under sachs interventions compared to the baseline condition.}
		Each panel compares the baseline order inferred on \texttt{cd3cd28} to the order inferred under the intervention. Baseline nodes are shown in \texttt{fliplow}; intervention nodes are colored by their pairwise flip fraction relative to the baseline.}
	\label{fig:sachs-intervention-order-lineups}
\end{figure}

==> figs/sachs-flip.tex <==
% Requires:
% \usepackage{subcaption}
% \usetikzlibrary{positioning,arrows.meta}

% ---------------------------------------------------------------------
% Colors and shared node styles
% ---------------------------------------------------------------------

\definecolor{fliplow}{RGB}{245,248,252}
\definecolor{flipmid}{RGB}{120,185,180}
\definecolor{fliphigh}{RGB}{0,95,92}

\newcommand{\dy}{0.78}
\newcommand{\xbase}{-1.6}
\newcommand{\xcond}{1.6}

\newcommand{\basenode}[3]{%
	\node[
	circle,
	minimum size=6.5mm,
	inner sep=1pt,
	fill=fliplow
	] (#1) at #2 {#3};
}

\newcommand{\colornodeat}[4]{%
	\pgfmathparse{#4 < 50 ? int(2*#4) : int(2*(#4-50))}
	\let\mixval\pgfmathresult
	\ifnum#4<50
	\node[
	circle,
	minimum size=6.5mm,
	inner sep=1pt,
	fill=fliplow!\mixval!flipmid
	] (#1) at #2 {#3};
	\else
	\node[
	circle,
	minimum size=6.5mm,
	inner sep=1pt,
	fill=flipmid!\mixval!fliphigh
	] (#1) at #2 {#3};
	\fi
}

% ---------------------------------------------------------------------
% Left panel: two inferred orders
% ---------------------------------------------------------------------

\newcommand{\OrderPanel}[2]{%
	\begin{tikzpicture}[font=\scriptsize]
		\node at (\xbase,0.55) {\texttt{cd3cd28}};
		\node at (\xcond,0.55) {#1};
		
		\BaselineOrder
		#2
		
		\path[-{Latex[length=1.4mm,width=0.7mm]}, line width=0.55pt]
		(b1) edge (b2) (b2) edge (b3) (b3) edge (b4) (b4) edge (b5)
		(b5) edge (b6) (b6) edge (b7) (b7) edge (b8) (b8) edge (b9)
		(b9) edge (b10) (b10) edge (b11);
		
		\path[-{Latex[length=1.4mm,width=0.7mm]}, line width=0.55pt]
		(c1) edge (c2) (c2) edge (c3) (c3) edge (c4) (c4) edge (c5)
		(c5) edge (c6) (c6) edge (c7) (c7) edge (c8) (c8) edge (c9)
		(c9) edge (c10) (c10) edge (c11);
	\end{tikzpicture}
}

\newcommand{\BaselineOrder}{%
	\basenode{b1}{(\xbase,0)}{PKA}
	\basenode{b2}{(\xbase,-1*\dy)}{PKC}
	\basenode{b3}{(\xbase,-2*\dy)}{Plc${}_{\gamma}$}
	\basenode{b4}{(\xbase,-3*\dy)}{PIP3}
	\basenode{b5}{(\xbase,-4*\dy)}{Erk}
	\basenode{b6}{(\xbase,-5*\dy)}{Jnk}
	\basenode{b7}{(\xbase,-6*\dy)}{Akt}
	\basenode{b8}{(\xbase,-7*\dy)}{PIP2}
	\basenode{b9}{(\xbase,-8*\dy)}{P38}
	\basenode{b10}{(\xbase,-9*\dy)}{Mek}
	\basenode{b11}{(\xbase,-10*\dy)}{Raf}
}

\newcommand{\OrderUzero}{%
	\colornodeat{c1}{(\xcond,0)}{PKC}{10}
	\colornodeat{c2}{(\xcond,-1*\dy)}{Erk}{30}
	\colornodeat{c3}{(\xcond,-2*\dy)}{PKA}{20}
	\colornodeat{c4}{(\xcond,-3*\dy)}{Mek}{60}
	\colornodeat{c5}{(\xcond,-4*\dy)}{Raf}{60}
	\colornodeat{c6}{(\xcond,-5*\dy)}{Jnk}{40}
	\colornodeat{c7}{(\xcond,-6*\dy)}{Plc${}_{\gamma}$}{40}
	\colornodeat{c8}{(\xcond,-7*\dy)}{PIP3}{40}
	\colornodeat{c9}{(\xcond,-8*\dy)}{P38}{40}
	\colornodeat{c10}{(\xcond,-9*\dy)}{PIP2}{40}
	\colornodeat{c11}{(\xcond,-10*\dy)}{Akt}{40}
}

\newcommand{\OrderGzero}{%
	\colornodeat{c1}{(\xcond,0)}{P38}{80}
	\colornodeat{c2}{(\xcond,-1*\dy)}{PIP2}{80}
	\colornodeat{c3}{(\xcond,-2*\dy)}{Mek}{70}
	\colornodeat{c4}{(\xcond,-3*\dy)}{Jnk}{80}
	\colornodeat{c5}{(\xcond,-4*\dy)}{Plc${}_{\gamma}$}{60}
	\colornodeat{c6}{(\xcond,-5*\dy)}{Raf}{50}
	\colornodeat{c7}{(\xcond,-6*\dy)}{Akt}{80}
	\colornodeat{c8}{(\xcond,-7*\dy)}{PIP3}{80}
	\colornodeat{c9}{(\xcond,-8*\dy)}{PKA}{80}
	\colornodeat{c10}{(\xcond,-9*\dy)}{PKC}{80}
	\colornodeat{c11}{(\xcond,-10*\dy)}{Erk}{60}
}

\newcommand{\OrderPsitect}{%
	\colornodeat{c1}{(\xcond,0)}{PIP2}{70}
	\colornodeat{c2}{(\xcond,-1*\dy)}{Plc${}_{\gamma}$}{30}
	\colornodeat{c3}{(\xcond,-2*\dy)}{PKA}{20}
	\colornodeat{c4}{(\xcond,-3*\dy)}{PIP3}{20}
	\colornodeat{c5}{(\xcond,-4*\dy)}{PKC}{30}
	\colornodeat{c6}{(\xcond,-5*\dy)}{Akt}{30}
	\colornodeat{c7}{(\xcond,-6*\dy)}{Jnk}{30}
	\colornodeat{c8}{(\xcond,-7*\dy)}{P38}{10}
	\colornodeat{c9}{(\xcond,-8*\dy)}{Erk}{40}
	\colornodeat{c10}{(\xcond,-9*\dy)}{Raf}{10}
	\colornodeat{c11}{(\xcond,-10*\dy)}{Mek}{10}
}

\newcommand{\OrderLy}{%
	\colornodeat{c1}{(\xcond,0)}{PKA}{0}
	\colornodeat{c2}{(\xcond,-1*\dy)}{Plc${}_{\gamma}$}{10}
	\colornodeat{c3}{(\xcond,-2*\dy)}{PKC}{10}
	\colornodeat{c4}{(\xcond,-3*\dy)}{PIP3}{0}
	\colornodeat{c5}{(\xcond,-4*\dy)}{Erk}{0}
	\colornodeat{c6}{(\xcond,-5*\dy)}{Jnk}{0}
	\colornodeat{c7}{(\xcond,-6*\dy)}{P38}{20}
	\colornodeat{c8}{(\xcond,-7*\dy)}{Akt}{10}
	\colornodeat{c9}{(\xcond,-8*\dy)}{PIP2}{10}
	\colornodeat{c10}{(\xcond,-9*\dy)}{Mek}{0}
	\colornodeat{c11}{(\xcond,-10*\dy)}{Raf}{0}
}

% ---------------------------------------------------------------------
% Right panel: fixed Sachs graph colored by pairwise flips
% ---------------------------------------------------------------------

\newcommand{\SachsFlipGraphSmall}{%
	\begin{tikzpicture}[font=\scriptsize]
		
		\colornodeat{pkc}{(0,4)}{PKC}{\pkcflip}
		\colornodeat{pka}{(0,2.4)}{PKA}{\pkaflip}
		\colornodeat{raf}{(1.7,2.4)}{Raf}{\rafflip}
		\colornodeat{jnk}{(-1.7,2.4)}{Jnk}{\jnkflip}
		\colornodeat{p38}{(-1.7,1.1)}{P38}{\pflip}
		\colornodeat{plcg}{(-2.4,0.2)}{Plc${}_{\gamma}$}{\plcgflip}
		\colornodeat{pip2}{(-3.3,-1.0)}{PIP2}{\piptwoflip}
		\colornodeat{pip3}{(-1.7,-1.0)}{PIP3}{\pipthreeflip}
		\colornodeat{akt}{(0,-1.0)}{Akt}{\aktflip}
		\colornodeat{erk}{(1.7,-1.0)}{Erk}{\erkflip}
		\colornodeat{mek}{(1.7,1.1)}{Mek}{\mekflip}
		
		\path[-{Latex[length=1.5mm,width=0.75mm]}, line width=0.6pt]
		(raf) edge[] (mek)
		(mek) edge[] (erk)
		
		(plcg) edge[bend right=10] (pip2)
		(plcg) edge[bend left=10] (pip3)
		
		(pip3) edge[] (pip2)
		(pip3) edge[] (akt)
		
		(pip2) edge[bend left=25] (pkc)
		
		(pkc) edge[] (raf)
		(pkc) edge[bend left=12] (mek)
		(pkc) edge[] (jnk)
		(pkc) edge[bend right=12] (p38)
		
		(pka) edge[] (raf)
		(pka) edge[] (mek)
		(pka) edge[bend left=10] (erk)
		(pka) edge[] (akt)
		(pka) edge[] (jnk)
		(pka) edge[] (p38);
		
	\end{tikzpicture}
}

% ---------------------------------------------------------------------
% Combined panel: orders left, graph right
% ---------------------------------------------------------------------

\newcommand{\CombinedSachsPanel}[4]{%
	% #1 condition label, #2 divtop, #3 order macro, #4 flip definitions
	#4
	\begin{tikzpicture}[font=\scriptsize]
		\node at (0,0) {\scalebox{0.64}{\OrderPanel{#1}{#3}}};
		\node at (5.0,-2.3) {\scalebox{0.58}{\SachsFlipGraphSmall}};
		\node at (2.6,0.8) {\textbf{#1}\quad $\divtop=#2$};
	\end{tikzpicture}
}

% ---------------------------------------------------------------------
% Figure
% ---------------------------------------------------------------------

\begin{figure}[t]
	\centering
	
	\begin{subfigure}{0.49\linewidth}
		\centering
		\CombinedSachsPanel{\texttt{u0126}}{0.265}{\OrderUzero}{%
			\def\pkaflip{20}\def\pkcflip{10}\def\plcgflip{40}\def\pipthreeflip{40}
			\def\erkflip{30}\def\jnkflip{40}\def\aktflip{40}\def\piptwoflip{40}
			\def\pflip{40}\def\mekflip{60}\def\rafflip{60}
		}
		\caption{MEK inhibition}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.49\linewidth}
		\centering
		\CombinedSachsPanel{\texttt{g0076}}{0.765}{\OrderGzero}{%
			\def\pkaflip{80}\def\pkcflip{80}\def\plcgflip{60}\def\pipthreeflip{80}
			\def\erkflip{60}\def\jnkflip{80}\def\aktflip{80}\def\piptwoflip{80}
			\def\pflip{80}\def\mekflip{70}\def\rafflip{50}
		}
		\caption{PKC inhibition}
	\end{subfigure}
	
	\vspace{0.6em}
	
	\begin{subfigure}{0.49\linewidth}
		\centering
		\CombinedSachsPanel{\texttt{psitect}}{0.235}{\OrderPsitect}{%
			\def\pkaflip{20}\def\pkcflip{30}\def\plcgflip{30}\def\pipthreeflip{20}
			\def\erkflip{40}\def\jnkflip{30}\def\aktflip{30}\def\piptwoflip{70}
			\def\pflip{10}\def\mekflip{10}\def\rafflip{10}
		}
		\caption{Phosphoinositide perturbation}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.49\linewidth}
		\centering
		\CombinedSachsPanel{\texttt{ly}}{0.191}{\OrderLy}{%
			\def\pkaflip{0}\def\pkcflip{10}\def\plcgflip{10}\def\pipthreeflip{0}
			\def\erkflip{0}\def\jnkflip{0}\def\aktflip{10}\def\piptwoflip{10}
			\def\pflip{20}\def\mekflip{0}\def\rafflip{0}
		}
		\caption{PI3K inhibition}
	\end{subfigure}
	
	\caption{\textbf{Order changes and graph-localized intervention effects under selected Sachs interventions.}
		Each panel shows the baseline order inferred on \texttt{cd3cd28} and the order inferred under the intervention, together with the fixed Sachs consensus graph. Baseline nodes are shown in \texttt{fliplow}; intervention and graph nodes are colored by pairwise flip fraction relative to the baseline.}
	\label{fig:sachs-combined-orders-graph}
\end{figure}

==> figs/sachs-intervention-stability.tex <==
% Expected data exports:
% - figs/texdata/sachs_intervention_abs.tsv
%   columns:
%   condition,
%   taborder_finetuned_mean, taborder_finetuned_se,
%   taborder_pretrained_mean, taborder_pretrained_se,
%   tabpfn_mean, tabpfn_se,
%   xgboost_mean, xgboost_se
% - figs/texdata/sachs_intervention_delta.tsv
%   columns:
%   perturbation,
%   taborder_finetuned_mean, taborder_finetuned_se,
%   taborder_pretrained_mean, taborder_pretrained_se,
%   tabpfn_mean, tabpfn_se,
%   xgboost_mean, xgboost_se
%
% Until these files are exported from the notebook, this figure falls back to
% a compile-safe placeholder.

\begin{figure}[t]
    \centering
    \IfFileExists{figs/texdata/sachs_intervention_abs.tsv}{%
    \IfFileExists{figs/texdata/sachs_intervention_delta.tsv}{%
        \begin{minipage}[t]{0.49\linewidth}
            \centering
            \begin{tikzpicture}
                \begin{axis}[
                    width=\linewidth,
                    height=4.6cm,
                    ybar,
                    bar width=5pt,
                    cycle list={
                        {fill=blue!55, draw=blue!55},
                        {fill=cyan!55!black, draw=cyan!55!black},
                        {fill=green!55!black, draw=green!55!black},
                        {fill=orange!80!black, draw=orange!80!black},
                    },
                    ymin=0,
                    xlabel={Condition},
                    ylabel={Mean source-z MAE},
                    symbolic x coords={iid,all\_direct\_parents\_randomized,all\_direct\_children\_randomized},
                    xtick=data,
                    xticklabel style={rotate=18,anchor=east,font=\scriptsize},
                    legend style={font=\scriptsize, draw=none, at={(0.5,1.02)}, anchor=south, legend columns=2},
                    title={(a) Absolute error},
                ]
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=condition, y=taborder_finetuned_mean, y error=taborder_finetuned_se, col sep=tab] {figs/texdata/sachs_intervention_abs.tsv};
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=condition, y=taborder_pretrained_mean, y error=taborder_pretrained_se, col sep=tab] {figs/texdata/sachs_intervention_abs.tsv};
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=condition, y=tabpfn_mean, y error=tabpfn_se, col sep=tab] {figs/texdata/sachs_intervention_abs.tsv};
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=condition, y=xgboost_mean, y error=xgboost_se, col sep=tab] {figs/texdata/sachs_intervention_abs.tsv};
                    \legend{\ourmethod{} (ft), \ourmethod{} (pt), \tabpfn, \xgboost}
                \end{axis}
            \end{tikzpicture}
        \end{minipage}\hfill
        \begin{minipage}[t]{0.49\linewidth}
            \centering
            \begin{tikzpicture}
                \begin{axis}[
                    width=\linewidth,
                    height=4.6cm,
                    ybar,
                    bar width=8pt,
                    cycle list={
                        {fill=blue!55, draw=blue!55},
                        {fill=cyan!55!black, draw=cyan!55!black},
                        {fill=green!55!black, draw=green!55!black},
                        {fill=orange!80!black, draw=orange!80!black},
                    },
                    ymin=0,
                    xlabel={Perturbation},
                    ylabel={$\Delta$ source-z MAE from IID},
                    symbolic x coords={parent,child},
                    xtick=data,
                    xticklabel style={font=\scriptsize},
                    title={(b) Degradation from IID},
                ]
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=perturbation, y=taborder_finetuned_mean, y error=taborder_finetuned_se, col sep=tab] {figs/texdata/sachs_intervention_delta.tsv};
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=perturbation, y=taborder_pretrained_mean, y error=taborder_pretrained_se, col sep=tab] {figs/texdata/sachs_intervention_delta.tsv};
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=perturbation, y=tabpfn_mean, y error=tabpfn_se, col sep=tab] {figs/texdata/sachs_intervention_delta.tsv};
                    \addplot+[error bars/.cd, y dir=both, y explicit]
                        table[x=perturbation, y=xgboost_mean, y error=xgboost_se, col sep=tab] {figs/texdata/sachs_intervention_delta.tsv};
                \end{axis}
            \end{tikzpicture}
        \end{minipage}
    }{%
        \fbox{%
            \parbox{0.95\linewidth}{%
                \vspace{0.4em}
                \centering
                \textbf{Sachs intervention stability figure placeholder.}\\
                Export the aggregated notebook results to\\
                \texttt{figs/texdata/sachs\_intervention\_abs.tsv} and
                \texttt{figs/texdata/sachs\_intervention\_delta.tsv}.\\
                The final figure should report absolute source-z MAE across IID,
                parent-perturbed, and child-perturbed settings, together with
                the corresponding degradation from IID.
                \vspace{0.4em}
            }%
        }%
    }}{%
        \fbox{%
            \parbox{0.95\linewidth}{%
                \vspace{0.4em}
                \centering
                \textbf{Sachs intervention stability figure placeholder.}\\
                Export the aggregated notebook results to\\
                \texttt{figs/texdata/sachs\_intervention\_abs.tsv} and
                \texttt{figs/texdata/sachs\_intervention\_delta.tsv}.\\
                The final figure should report absolute source-z MAE across IID,
                parent-perturbed, and child-perturbed settings, together with
                the corresponding degradation from IID.
                \vspace{0.4em}
            }%
        }%
    }
    \caption{\textbf{Intervention stability on Sachs.}
    Absolute performance on Sachs is similar across methods, but \ourmethod exhibits a smaller degradation relative to its own IID performance under intervention. We therefore interpret the result as evidence of intervention stability rather than uniformly better absolute predictive accuracy.}
    \label{fig:sachs-intervention-stability}
\end{figure}


==> figs/sachs-minigraph.tex <==
\begin{wrapfigure}{r}{0.52\textwidth}
	\centering
	
	\begin{subfigure}{0.48\linewidth}
		\centering
		\def\pkaflip{20}\def\pkcflip{10}\def\plcgflip{40}\def\pipthreeflip{40}
		\def\erkflip{30}\def\jnkflip{40}\def\aktflip{40}\def\piptwoflip{40}
		\def\pflip{40}\def\mekflip{60}\def\rafflip{60}
		\scalebox{0.42}{\SachsFlipGraph{\texttt{u0126}}{0.265}} %todo remove the args
		\caption{MEK inhibition (\texttt{u0126})}
	\end{subfigure}
 
	
	\caption{\textbf{Differences in causal-order positionings under Sachs interventions.}
		Nodes are colored by pairwise flip fraction relative to \texttt{cd3cd28}; edges show the fixed consensus graph. The topological divergence is $\divtop=0.265$.}
	\label{fig:sachs-intervention-graph-flips-wrap}
\end{wrapfigure}

==> figs/sachs-rank-graph.tex <==
\begin{figure}[t]
	\centering
	
	% Row 1
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsActivatorTwo
		\ShowSachsRankICAM
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28\_icam2}}{0.235}}
		\caption{\textbf{\texttt{cd3cd28\_icam2}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsActivatorThree
		\ShowSachsRankPMA
		\scalebox{0.5}{\SachsRankGraph{\texttt{pma}}{--}}
		\caption{\textbf{\texttt{pma}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSix
		\ShowSachsRankUzero
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28\_u0126}}{0.265}}
		\caption{\textbf{\texttt{cd3cd28\_u0126}.}}
	\end{subfigure}
	
	\vspace{0.7em}
	
	% Row 2
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSix
		\ShowSachsActivatorTwo
		\ShowSachsRankICAMUzero
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28icam2\_u0126}}{--}}
		\caption{\textbf{\texttt{cd3cd28icam2\_u0126}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFive
		\ShowSachsRankAktInhib
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28\_aktinhib}}{0.294}}
		\caption{\textbf{\texttt{cd3cd28\_aktinhib}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFive
		\ShowSachsActivatorTwo
		\ShowSachsRankICAMAktInhib
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28icam2\_aktinhib}}{0.132}}
		\caption{\textbf{\texttt{cd3cd28icam2\_aktinhib}.}}
	\end{subfigure}
	
	\vspace{0.7em}
	
	% Row 3
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFour
		\ShowSachsRankGzero
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28\_g0076}}{0.765}}
		\caption{\textbf{\texttt{cd3cd28\_g0076}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorFour
		\ShowSachsActivatorTwo
		\ShowSachsRankICAMGzero
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28icam2\_g0076}}{0.544}}
		\caption{\textbf{\texttt{cd3cd28icam2\_g0076}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSeven
		\ShowSachsRankLy
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28\_ly}}{0.191}}
		\caption{\textbf{\texttt{cd3cd28\_ly}.}}
	\end{subfigure}
	
	\vspace{0.7em}
	
	% Row 4
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorSeven
		\ShowSachsActivatorTwo
		\ShowSachsRankICAMLy
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28icam2\_ly}}{--}}
		\caption{\textbf{\texttt{cd3cd28icam2\_ly}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorEight
		\ShowSachsRankPsitect
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28\_psitect}}{0.235}}
		\caption{\textbf{\texttt{cd3cd28\_psitect}.}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\linewidth}
		\centering
		\ResetSachsInterventions
		\ShowSachsInhibitorEight
		\ShowSachsActivatorTwo
		\ShowSachsRankICAMPsit
		\scalebox{0.5}{\SachsRankGraph{\texttt{cd3cd28icam2\_psit}}{--}}
		\caption{\textbf{\texttt{cd3cd28icam2\_psit}.}}
	\end{subfigure}
	
	\caption{\textbf{Rank shifts in causal-order positionings under Sachs experimental conditions.}
		Nodes are colored by signed rank shift relative to \texttt{cd3cd28}; golden nodes move later in the inferred order, while blue nodes move earlier. Edges show the fixed consensus graph, and activator/inhibitor markers indicate the corresponding experimental perturbations.}
	\label{fig:sachs-all-intervention-graph-rankshifts}
\end{figure}

==> figs/table-sachs-info.tex <==
\begin{table}[h!] 
	\caption{\textbf{Sachs Dataset Conditions and Corresponding Biological Interventions}. The \texttt{cd3cd28} condition is commonly treated as an observational proxy, although it still involves TCR/CD28 stimulation and is therefore not a strictly unperturbed observational distribution.}
	\label{tab:sachs-interventions}  \vspace*{1em}
	\normalsize
	\begin{tabular}{ll}
		\toprule
		Condition $\cond$ & Intervention  \\
		\midrule
		\texttt{cd3cd28}$(\obs)$
		& TCR/CD28 stimulation (observational proxy) \\
		
		\texttt{cd3cd28\_icam2}
		& TCR/CD28 + ICAM-2 co-stimulation \\
		
		\texttt{cd3cd28\_u0126}
		& MEK inhibition \\
		
		\texttt{cd3cd28\_aktinhib}
		& Akt inhibition \\
		
		\texttt{cd3cd28icam2\_aktinhib}
		& Akt inhibition + ICAM-2 co-stimulation \\
		
		\texttt{cd3cd28\_g0076}
		& PKC inhibition \\
		
		\texttt{cd3cd28icam2\_g0076}
		& PKC inhibition + ICAM-2 co-stimulation \\
		
		\texttt{cd3cd28\_ly}
		& PI3K inhibition (upstream of PIP3/Akt) \\
		
		\texttt{cd3cd28\_psitect}
		& Phosphoinositide perturbation (PIP2/PIP3 axis) \\\bottomrule
	\end{tabular}\vspace*{1em}
\end{table}



==> sections/figs/ablation_ordergap.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			rankplot,
			pretty line,
			pretty labelshift,
			cycle list name=topic-line,
			xlabel={Topological divergence},
			ylabel={Negative log-likelihood},
			xmin=0.0, xmax=0.52,
			ymin=0.05, ymax=0.30,
			legend style={
				at={(0.5,1.05)},
				anchor=south,
				legend columns=2,
				draw=none
			},
			]
			
			% Learned NLL
			\addplot+[
			mark=*,
			]
			coordinates {
				(0.02, 0.063)
				(0.25, 0.15)
				(0.35, 0.20)
				(0.45, 0.24)
				(0.50, 0.266)
			};
			\addlegendentry{NLL (learned)}
			
			% Oracle NLL
			\addplot+[
			mark=square*,
			]
			coordinates {
				(0.02, 0.058)
				(0.25, 0.135)
				(0.35, 0.20)
				(0.45, 0.24)
				(0.50, 0.279)
			};
			\addlegendentry{NLL (oracle)}
			
			% Annotations on x-axis
			\node[anchor=north west, font=\scriptsize] 
			at (axis cs:0.02,0.05) {near-oracle};
			
			\node[anchor=north east, font=\scriptsize] 
			at (axis cs:0.5,0.05) {large div.};
			
		\end{axis}
	\end{tikzpicture}
	
	\caption{\textbf{Likelihood vs. Topological Divergence}. Negative log-likelihood increases as the inferred order deviates from the true causal ordering.}
	\label{fig:nll_vs_divergence}
\end{figure}

==> sections/sachs_intervention_stability.tex <==
\paragraph{Unknown Biological Interventions.} \input{figs/sachs-intervention-stability}
We finally revisit the Sachs benchmark in a setting where the intervention target is not given to the predictor. For each Sachs environment, we split observations into train and test rows, predict held-out targets under the native test distribution, and then repeat evaluation after perturbing either all direct parents or all direct children of the target in the test rows. We aggregate source-z MAE over environment-seed runs and compare the pretrained and fine-tuned variants of \ourmethod against \tabpfn{} and \xgboost.

Figure~\ref{fig:sachs-intervention-stability} shows that the methods are broadly similar in absolute performance across the three settings. The main distinction is that \ourmethod exhibits a smaller error increase relative to its own IID performance under both parent and child perturbations. We therefore interpret the Sachs result as evidence of intervention stability rather than uniformly better absolute prediction.

At the same time, a small intervention delta is not meaningful in isolation, since a model with weaker IID fit may also appear stable simply because it is less responsive overall. For this reason, we report absolute error and degradation from IID side by side. Under this reading, the Sachs experiment supports a tradeoff interpretation: \ourmethod is not uniformly dominant in absolute error, but it appears less sensitive to perturbations that break environment-specific dependencies.

